Solving the minimum labeling global cut problem by mathematical programming

Let G = (V, E, L) be an edge-labeled graph such that V is the set of vertices, E is the set of edges, L is the set of labels (colors) and each edge e \in E has a label l(e) associated; The goal of the minimum labeling global cut problem (MLGCP) is to find a subset L \subseteq L of labels such that G = (V, E , L\L ) is not connected and |L| is minimized. This work proposes three new mathematical formulations for the MLGCP as well as branch-and-cut algorithms to solve them. The computational experiments showed that the proposed methods are able to solve small to average sized instances in a reasonable amount of time.

==> 4_heuristic.tex <==
\section{Heurísticas para o MLCP}

\subsection{Representação da solução}

Um dos grande problemas da representação de uma solução $G$ para o MLCP é garantir que a coleção de cores que a define seja de fato um corte. Para isto definimos o par de partições $P^G =\{P^G_l,P^G_r\}$, onde $P^G_l$ representa o conjunto de vértices da partição esquerda e $P^G_r$ o conjunto dos vértices da partição direita. Se $\left|P^G_l \right| > 0$ e $\left|P^G_l\right| > 0$ então temos a garantia de um corte válido. Ainda para representar a solução $G$ temos o conjunto $L^G=\{L_{i,j} | i \in P^G_l, j \in P^G_r\}$, sendo o custo da solução $G$ computada por $custo(G)=\left|L^G\right|$.

\subsection {Movimentos de Vizinhança}

Para a realização dos procedimentos de Busca Local propomos dois movimentos de vizinhança. Em todos os procedimentos de movimentação de vizinhança, é considerada uma solução prévia viável $G'$ formada por um par de partições $P^{G'}$ válido.

\medskip

\noindent \textbf{\textit{Change-partition}}: move um vértice $v \in P^{G'}_l$  para a partição $P^{G'}_r$ ou um vértice $v \in P^{G'}_r$ para a partição $P^{G'}_l$. Atualizando o conjunto de cores do corte $L^G$. Figura \ref{fig:movements}(a) apresenta este movimento.

\noindent \textbf{\textit{Interchange-partition}}: move um vértice $v \in P^{G'}_l$  para a partição $P^{G'}_r$ e um vértice $u \in P^{G'}_r$ para a partição $P^{G'}_l$. Atualizando o conjunto de cores do corte $L^G$. Figura \ref{fig:movements}(a) apresenta este movimento.

\subsection{Estrutura de dados auxiliar}

A avaliação de todos os movimentos de vizinhança propostos neste trabalho é composta pela atualização do conjunto $L^G$. Assim, com o objetivo de acelerar a fase de busca local, definimos uma estrutura que indica a frequência de cada cor contida nas arestas do corte representado pela específica solução, esta estrutura permite a avaliação de cada movimento em tempo constante ($O(1)$). 


\begin{figure}[h]
    \centering
        \includegraphics[scale=0.65]{figura/colorCounter.pdf}
    \caption{(a)Solution $G$ with $\left|L^G\right| = 3$. (b) Create solution $G'$ with a Change-partition moviment. (c) Remove the B color of L^{G'} (B  count set to zero) }
    \label{fig:movements}
\end{figure}



Seja $G'$ uma solução formada pela coleção $\mathcal{B}$ de \textit{biclusters}. A Matriz de Edições $M$ para $G'$ é definida do seguinte modo. Uma entrada $M(v,B)$, para um vértice $v\in V_1$ e um \textit{bicluster} $B\in\mathcal{B}$, é dado por:






==> 4_inst.tex <==
\section{\textit{Benchmark}}

Para os experimentos realizados, utilizamos os GARs gerados de forma aleatória por \cite{Cerulli:2005}. Para cada $n=|V|= 50, 100, 200$, as instâncias possuem 90 grafos-problema. Cada conjunto consiste em $9$ grupos de instâncias com distintas dimensões, sendo cada grupo definido por uma combinação entre $|L|=\{\frac{n}{2};n;\frac{5n}{4}\}$ e $d=\{ld=0,2; md=0,5; hd=0,8\}$, \textit{d} representando a densidade do grafo. Cada grupo possui $10$ instâncias distintas de mesma dimensão.

Para cada grafo-instância, foram gerados três cenários para os custos de remoção dos rótulos. No primeiro cenário, denominado \textit{unicost}, todos os rótulos possuem custo de remoção igual a $1$; no segundo cenário, denominado \textit{random}, o custo de remoção de cada rótulo foi escolhido de forma aleatória no intervalo $[0,01 - 0,99]$; e no terceiro cenário, denominado \textit{normal}, os custos remoção dos rótulos foram gerados de forma aleatória no intervalo $[0,01 - 0,99]$, mas obedecendo uma distribuição normal com média $0,5$ e $\sigma^2 = 0,20$. A Figura \ref{fig:random} traz o histograma dos custos de remoção dos rótulos gerados no cenário \textit{normal} (a), e no cenário \textit{random} (b), para uma instância com $|L|=100$.


\begin{figure}[h]
	\centering
		\includegraphics[scale=0.65]{figuras/random.png}
	\caption{Histograma do custo de remoção dos rótulos gerado aleatoriamente}
	\label{fig:random}
\end{figure}

==> tabelas/normal.100.tex <==
\begin{table}[htb]
	\centering
	\caption{Resultados computacionais para instâncias com $|V| = 100$,}
  \vspace{3mm}	
  \setlength{\tabcolsep}{5,6pt}
	
	\footnotesize
	\begin{tabular}{r l r c r r r r c r r r r }


	\hline
	\multicolumn{3}{c}{\bif{Instâncias}} & & \multicolumn{4}{ c }{\bif{PART$_2$}} & & \multicolumn{4}{ c }{\bif{EAC}}\\
	
	\cline{1-3} \cline{5-8} \cline{10-13}
	
	\bif{$|L|$} & \bif{d} & \bif{Opt} & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  \\

	
	\hlinewd{1,5pt}	
	

    &  ld & 6,2 & & 10 & 0,9 & 0 & 83,2 & & 10 & 0,03 & 0 & 47,7 \\
25  &  md & 16,5 & & 10 & 0,7 & 0 & 91,0 & & 10 & 0,05 & 0 & 50,6 \\
    &  hd & 21 & & 10 & 0,4 & 0 & 86,2 & & 10 & 0,03 & 0 & 72,9 \\

    &    \\

    &  ld & 6,8 & & 10 & 2,4 & 0 & 83,7 & & 10 & 0,2 & 0 & 57,2 \\
50  &  md & 22,2 & & 10 & 5,6 & 0 & 93,4 & & 10 & 3,4 & 0 & 77,2 \\
    &  hd & 33,1 & & 10 & 4,7 & 0 & 95,7 & & 10 & 3,9 & 0 & 77,1 \\

    &    \\

    &  ld & 7,2 & & 10 & 2,1 & 0 & 84,3 & & 10 & 2,2 & 0 & 65,7 \\
100 &  md & 26,5 & & 10 & 9,3 & 0 & 95,2 & & 9 & 850,7 & 0,5 & 85,5 \\
    &  hd & 45,2 & & 10 & 22,4 & 0 & 96,4 & & 4 & 2828,6 & 4,0 & 87,5 \\

    &    \\

    &  ld & 7,2 & & 10 & 3,1 & 0 & 84,1 & & 10 & 6,0 & 0 & 64,5 \\
125 &  md & 27,1 & & 10 & 36,0 & 0 & 95,0 & & 6 & 2195,4 & 6,2 & 87,4 \\
    &  hd & 45,2 & & 10 & 22,4 & 0 & 96,4 & & 4 & 2828,2 & 4,0 & 87,5 \\

	\hline	
	\end{tabular}
	\label{tab:n100}
\end{table}


==> tabelas/normal.200.tex <==
\begin{table}[htb]
	\centering
	\caption{Resultados computacionais no cenário \textit{normal} para instâncias com $|V| = 200$.}
  \vspace{3mm}	
  \setlength{\tabcolsep}{5.6pt}
	
	\footnotesize
	\begin{tabular}{r l r c r r r r c r r r r c r r r r }


	\hline
	\multicolumn{3}{c}{\bif{Instâncias}} & & \multicolumn{4}{c}{\bif{EP3}} & & \multicolumn{4}{ c }{\bif{PART$_2$}} & & \multicolumn{4}{ c }{\bif{EAC}}\\
	
	\cline{1-3} \cline{5-8} \cline{10-13} \cline{15-18}
	
	\bif{$|L|$} & \bif{d} & \bif{Opt} & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  \\

	
	\hlinewd{1.5pt}	
	
		
    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
100 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

    &    \\

    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
200 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

    &    \\

    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
250 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

	\hline	
	\end{tabular}
	\label{tab:n200}
\end{table}

==> tabelas/normal.50.tex <==
\begin{table}[htb]
	\centering
	\caption{Resultados computacionais no cenário \textit{normal} para instâncias com $|V| = 50$.}
  \vspace{3mm}	
  \setlength{\tabcolsep}{5.6pt}
	
	\footnotesize
	\begin{tabular}{r l r c r r r r c r r r r c r r r r }


	\hline
	\multicolumn{3}{c}{\bif{Instâncias}} & & \multicolumn{4}{c}{\bif{EP3}} & & \multicolumn{4}{ c }{\bif{PART$_2$}} & & \multicolumn{4}{ c }{\bif{EAC}}\\
	
	\cline{1-3} \cline{5-8} \cline{10-13} \cline{15-18}
	
	\bif{$|L|$} & \bif{d} & \bif{Opt} & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  \\

	
	\hlinewd{1.5pt}	
	
		
    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
 25 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

    &    \\

    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
 50 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

    &    \\

    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
 62 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

	\hline	
	\end{tabular}
	\label{tab:n50}
\end{table}

==> tabelas/random.100.tex <==
\begin{table}[htb]
	\centering
	\caption{Resultados computacionais no cenário \textit{random} para instâncias com $|V| = 100$.}
  \vspace{3mm}	
  \setlength{\tabcolsep}{5.6pt}
	
	\footnotesize
	\begin{tabular}{r l r c r r r r c r r r r c r r r r }


	\hline
	\multicolumn{3}{c}{\bif{Instâncias}} & & \multicolumn{4}{c}{\bif{EP3}} & & \multicolumn{4}{ c }{\bif{PART$_2$}} & & \multicolumn{4}{ c }{\bif{EAC}}\\
	
	\cline{1-3} \cline{5-8} \cline{10-13} \cline{15-18}
	
	\bif{$|L|$} & \bif{d} & \bif{Opt} & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  \\

	
	\hlinewd{1.5pt}	
	
		
    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
 50 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

    &    \\

    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
100 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

    &    \\

    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
125 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

	\hline	
	\end{tabular}
	\label{tab:r100}
\end{table}

==> tabelas/random.200.tex <==
\begin{table}[htb]
	\centering
	\caption{Resultados computacionais no cenário \textit{random} para instâncias com $|V| = 200$.}
  \vspace{3mm}	
  \setlength{\tabcolsep}{5.6pt}
	
	\footnotesize
	\begin{tabular}{r l r c r r r r c r r r r c r r r r }


	\hline
	\multicolumn{3}{c}{\bif{Instâncias}} & & \multicolumn{4}{c}{\bif{EP3}} & & \multicolumn{4}{ c }{\bif{PART$_2$}} & & \multicolumn{4}{ c }{\bif{EAC}}\\
	
	\cline{1-3} \cline{5-8} \cline{10-13} \cline{15-18}
	
	\bif{$|L|$} & \bif{d} & \bif{Opt} & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  \\

	
	\hlinewd{1.5pt}	
	
		
    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
100 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

    &    \\

    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
200 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

    &    \\

    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
250 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

	\hline	
	\end{tabular}
	\label{tab:r200}
\end{table}

==> tabelas/random.50.tex <==
\begin{table}[htb]
	\centering
	\caption{Resultados computacionais no cenário \textit{random} para instâncias com $|V| = 50$.}
  \vspace{3mm}	
  \setlength{\tabcolsep}{5.6pt}
	
	\footnotesize
	\begin{tabular}{r l r c r r r r c r r r r c r r r r }


	\hline
	\multicolumn{3}{c}{\bif{Instâncias}} & & \multicolumn{4}{c}{\bif{EP3}} & & \multicolumn{4}{ c }{\bif{PART$_2$}} & & \multicolumn{4}{ c }{\bif{EAC}}\\
	
	\cline{1-3} \cline{5-8} \cline{10-13} \cline{15-18}
	
	\bif{$|L|$} & \bif{d} & \bif{Opt} & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  & & \bif{O} &
	\multicolumn{1}{c}{\bif{t (s)}}  &
	\multicolumn{1}{c}{\bif{gap}}  &
	\multicolumn{1}{c}{\bif{gapr}}  \\

	
	\hlinewd{1.5pt}	
	
		
    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
 25 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

    &    \\

    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
 50 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

    &    \\

    & ld & 11,9 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 & & 7  & 4842 & 40,2 & 30,2 \\
 62 & md & 5,4  & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   & & 8  & 325  &  5,5 & 21   \\
    & hd & 4,0  & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 & & 9  & 89   &  1,7 & 12,1 \\

	\hline	
	\end{tabular}
	\label{tab:r50}
\end{table}
